Weyl channels for multipartite systems

Quantum channels, a subset of quantum maps, describe the unitary and non-unitary evolution of quantum systems. We study a generalization of the concept of Pauli maps to the case of multipartite high dimensional quantum systems through the use of the Weyl operators. The condition for such maps to be valid quantum channels, i.e. complete positivity, is derived in terms of Fourier transform matrices. From these conditions, we find the extreme points of this set of channels and identify an elegant algebraic structure nested within them. In turn, this allows us to expand upon the concept of "component erasing channels" introduced in earlier work by the authors. We show that these channels are completely characterized by elements drawn of finite cyclic groups. An algorithmic construction for such channels is presented and the smallest subsets of erasing channels which generate the whole set are determined.

==> WeylGenerators.tex <==
\subsection{Generators}

==> generators_proof.tex <==
\section{Proof Theorems for Generators of WCE channels}\label{app:generators}
\textbf{Theorem 2:} If $G$ is an abelian group of order $r = p_1^{n_1}p_2^{n_2} \cdots p_m^{n_m}$, then the generators of $G$ are the subgroups $N \leq G$ such that $G/N$ is cyclic and has order $p_i^k$ (with $0 \leq k \\leq n_i$, for some $i \in \{1,\cdots, m\}$ \\

\textbf{Proof:} We first notice that if $|G/N|$ is not a prime power, then $N$ can not be a generator, which means that this condition is necessary. 
That is, we assume that $|G/N|$ can be divided by two distinct primes $p_i$ and $p_j$. 
By Cauchy's theorem in group theory, this implies that $G/N$ has a subgroup of order $p_i$ and one of order $p_j$. 
Then, the correspondence theorem says that these subgroups are of the form $H_1 / N$, $H_j/N$ with $N < H_i, H_j \leq G$.
 Furthermore, the intersection of these subgroups must have an order that divides $p_i$ and $p_j$, so we conclude that they intersect trivially.
That is, $H_i/N \cap H_j/N = \{N\}$, so $(H_i \cap H_j)/N = \{N\}$ and we conclude that $H_i \cap H_j = N$. 
Therefore, we found two subgroups different to $N$ whose intersection is $N$ and we conclude that $N$ is not a generator. \\

Now we see that $G/N$ has to be cyclic for $N$ to be a generator.
To see this, notice that because of the fundamental theorem of finite abelian groups, $G/N$ is isomorphic to a product of the form $C_{i_1} \oplus C_{i_2} \oplus \cdots \oplus C_{i_r}$, where $C_{i_j}$ is the cyclic group of order $i_j$. 
If we assume that $G/N$ isn't cyclic, this product must include at least two factors. 
Therefore, if we define $K = C_{i_2} \oplus \cdots \oplus C_{i_r}$, the group $G/N$ is isomorphic to a group of the form $C_{i_1} \oplus K$.
Therefore, we can consider the subgroups $C_{i_1}' = \{(g, 0_k) \; | \; g \in C_{i_1}\}$, $K' = \{(0_{C_{i_1}},g) \; | \; g \in K\}$ of $G/N$, whose intersection is clearly trivial. 
Hence, we have found two subsets of $G/N$ whose intersection is trivial, and by the correspondence theorem, they can be written as $H_1/N, H_2/N$ where $N < H_1,H_2 \leq G$, with $H_1/N \cap H_2/N = \{N\}$. Just as before, this leads to the conclusion that $N$ is not a generator. \\

Now we prove that subgroups $N$ with these characteristics are generators.
Take $N \leq G$ such that $|G/N| = p_i^k$ and $G/N$ is cyclic. 
This implies that $G/N = \langle N \oplus g \rangle$ for some element $N \oplus g \in G/N$ of order $p_i^k$. 
Then, because of the properties of cyclic groups, all subgroups of $G/N$ are of the form $\langle p_i^s (N \oplus g) \rangle$ for $s \in \{0,1, \cdots, k-1\}$ (when $s = k$, the subgroup is the trivial $\{N\}$). 
The intersection of all these subgroups (omitting the trivial) is $\langle p_i^{k-1}(N \oplus g) \rangle$, which is non trivial. 

Then, if we define $H_1, H_2, \cdots, H_l$ as the subgroups of $G$ that properly contain $N$ (that is, the elements of $Sg(N)$). 
According to the correspondence theorem, each of these subgroups can be related biyectively with a subgroup $H_i /N$ of $G/N$. 
Therefore, the intersection of all these $H_i/N$ is equal to $\langle (N \oplus g)^{p_i^{k-1}} \rangle$ 
and hence $(\cap_{i=0}^l H_i)/N = (Ng)^{p_i^{k-1}}$.
Because this result is not the trivial $\{N\}$, we conclude that $\cap_{i=0}^l H_i$ is a set that contains $N$ and more elements,
which means that $\cap_{H \in Sg(N)} H \neq N$ and therefore $N$ is a generator. $\blacksquare$ \\

\textbf{Theorem 3:} \textit{$N \leq \mathbb{Z_d} \oplus \mathbb{Z_d}$ is a generator if and only if $N = \{(p,q) \; | \; pn-qm = 0\} := S_{mn}$ for some $(m,n)$ and $\dfrac{d^2}{|A|}$ is a prime power.} \\ 

\textbf{Proof:} We use theorem 2 and therefore only need to prove that a subgroup $N \leq \mathbb{Z_d} \oplus \mathbb{Z_d}$ has the property that $(\mathbb{Z_d} \oplus \mathbb{Z_d}) / N$ is 
cyclic if and only if $N$ has the form of $S_{mn}$ for some $(m,n)$. \\

We begin by defining a function $\Phi_{mn}: \mathbb{Z}_d \times \mathbb{Z}_d \rightarrow \mathbb{Z}_d$ given by $\Phi_{mn}(p,q) = pn-qm$. 

Notice that this function is an homomorphism, because clearly $\Phi( (p,q) \oplus (p',q') ) = \Phi((p,q)) \oplus \Phi((p',q'))$. 
Furthermore, $S_{mn}$ is the kernel of $\Phi_{mn}$, that is $S_{mn} = Ker(\Phi_{mn})$. 
Then, using the first isomorphism theorem, we conclude that $(\mathbb{Z}_d \oplus \mathbb{Z}_d)/Ker(\Phi_{mn})$ is isomorphic to $Im(\Phi_{mn})$.
But $Im(\Phi_{mn})$ is a subgroup of $\mathbb{Z}_d$ and is therefore cyclic, which means that $(\mathbb{Z}_d \oplus \mathbb{Z}_d)/N$ is cyclic. \\

For the converse, we assume that $(\mathbb{Z}_d \oplus \mathbb{Z}_d)/N$ is cyclic, and let's say that $|(\mathbb{Z}_d \oplus \mathbb{Z}_d)/N| = l$,
Then, the elements of $(\mathbb{Z}_d \oplus \mathbb{Z}_d)/N$ are of the form
$\{N, N \oplus g, N \oplus 2g, \cdots, N \oplus (l-1)g\}$, for some element $g \in  mathbb{Z}_d \oplus \mathbb{Z}_d$ with order $l$, and together they form a partition of $\mathbb{Z}_d \oplus \mathbb{Z}_d$. Further, notice that $l$ must divide $d$, since all elements of $\mathbb{Z}_d \oplus \mathbb{Z}_d$ give as a result $(0,0)$ when added $d$ times.
 
Then, we define a function $\Phi: \mathbb{Z}_d \oplus \mathbb{Z}_d \rightarrow \mathbb{Z}_d$ such that if $x \in N \oplus kg$, we set $\Phi(x) = \dfrac{kd}{l}$. This function is clearly a morphism from $\mathbb{Z}_d \oplus \mathbb{Z}_d$ to $\mathbb{Z}_d$, since given $x \in N \oplus kg$ and $y \in N \oplus jg$, then $x+y \in N \oplus (k+j)g$. 

Finally ,  since $\Phi$ is a morphism from $\mathbb{Z}_d \oplus \mathbb{Z}_d$ to $\mathbb{Z}_d$, then for any $(p,q) \in \mathbb{Z}_d \oplus \mathbb{Z}_d$, we have that $\Phi(p,q) = p \Phi((1,0)) + q \Phi((0,1))$ and naming $n :=  \Phi((1,0))$, $m =  -\Phi((0,1))$, we conclude that $\Phi(p,q) = pn - qm$. Therefore, since any element in $N$ is mapped to $0$ when applying $\Phi$ (and no other elements are), we conclude that  $N$ has the form $\{(p,q) \; | \; pn-qm=0 \}$. $\blacksquare$ \\


\tbnote{Quitar probablemente la prueba del 3, pues es un caso especial de la del 4}.


\textbf{Theorem 4:} $N \leq \bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$ is a generator if and only if $N = \{(\vec{p},\vec{q}) \; | \; \vec{p} \cdot \vec{n}- \vec{q} \cdot \vec{m} = 0\} := S_{\vec{m} \vec{n}}$ for some $(\vec{m},\vec{n})$ and $\dfrac{D^2}{|N|}$ is a prime power. Where $\vec{p} \cdot \vec{n}$ is defined as $p_1 n_1 + p_2 n_2 + \cdots + p_Nn_N$.  \\

\textbf{Proof:} We use theorem 2 and therefore only need to prove that a subgroup $N \leq \bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$ has the property that $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})/ N$ is 
cyclic if and only if $N$ has the form of $S_{\vec{m} \vec{n}}$ for some $(\vec{m} \vec{n})$. \\

We begin by defining a function $\Phi_{\vec{m} \vec{n}}: \bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})\rightarrow \mathbb{Z}_D$ given by $\Phi_{\vec{m} \vec{n}}((\vec{p},\vec{q})) = \vec{p} \cdot \vec{n}- \vec{q} \cdot \vec{m}$. 

Notice that this function is an homomorphism, because clearly $\Phi( (\vec{p},\vec{q}) \oplus (\vec{p'},\vec{q'}) ) = \Phi( (\vec{p},\vec{q})) \oplus \Phi( (\vec{p'},\vec{q'}))$. 
Furthermore, $S_{\vec{m} \vec{n}}$ is the kernel of $\Phi_{\vec{m} \vec{n}}$, that is $S_{\vec{m} \vec{n}} = Ker(\Phi_{\vec{m} \vec{n}})$. 
Then, using the first isomorphism theorem, we conclude that $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i}) /Ker(\Phi_{\vec{m} \vec{n}})$ is isomorphic to $Im(\Phi_{mn})$.
But $Im(\Phi_{\vec{m} \vec{n}})$ is a subgroup of $\mathbb{Z}_D$ and is therefore cyclic, which means that $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})/N$ is cyclic. \\

For the converse, we assume that $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i}) /N$ is cyclic, and let's say that $|\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i}) /N| = l$,
Then, the elements of $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i}) /N$ are of the form
$\{N, N \oplus g, N \oplus 2g, \cdots, N \oplus (l-1)g\}$, for some element $g \in  \bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$ with order $l$, and together they form a partition of $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$. Further, notice that $l$ must divide $D$, since all elements of $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$ give as a result $(\vec{0},\vec{0})$ when added $D$ times.
 
Then, we define a function $\Phi: \bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i}) \rightarrow \mathbb{Z}_D$ such that if $x \in N \oplus kg$, we set $\Phi(x) = \dfrac{kD}{l}$. This function is clearly a morphism from $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$ to $\mathbb{Z}_D$, since given $x \in N \oplus kg$ and $y \in N \oplus jg$, then $x+y \in N \oplus (k+j)g$. 

Finally ,  since $\Phi$ is a morphism from $\bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$ to $\mathbb{Z}_D$, then for any $(\vec{p},\vec{q}) \in \bigoplus_{i=1}^N (\mathbb{Z}_{d_i} \oplus \mathbb{Z}_{d_i})$, we have that $\Phi(\vec{p},\vec{q}) = p_1 \Phi((\vec{e_1},0)) + p_2 \Phi((\vec{e_2},0)) + \cdots + p_N \Phi((\vec{e_N},0)) + q_1 \Phi((0,\vec{e}_1)) + q_2 \Phi((0,\vec{e_2})) + \cdots + q_N \Phi((0,\vec{e_N}))$, and naming $n_i :=  \Phi((\vec{e}_i,0))$, $m_i =  -\Phi((0,\vec{e}_i))$, we conclude that $\Phi((\vec{p},\vec{q})) = \vec{p} \cdot \vec{n} - \vec{q}\cdot \vec{m}$. Therefore, since any element in $N$ is mapped to $0$ when applying $\Phi$ (and no other elements are), we conclude that  $N$ has the form $\{(\vec{p}, \vec{q}) \; | \; \vec{p} \cdot \vec{n} - \vec{q}\cdot \vec{m}=0 \}$. $\blacksquare$. \\
